Helpful assistant or fruitful facilitator? Investigating how personas affect language model behavior

One way to personalize and steer generations from large language models (LLM) is to assign a persona: a role that describes how the user expects the LLM to behave (e.g., a helpful assistant, a teacher, a woman). This paper investigates how personas affect diverse aspects of model behavior. We assign to seven LLMs 162 personas from 12 categories spanning variables like gender, sexual orientation, and occupation. We prompt them to answer questions from five datasets covering objective (e.g., questions about math and history) and subjective tasks (e.g., questions about beliefs and values). We also compare persona's generations to two baseline settings: a control persona setting with 30 paraphrases of "a helpful assistant" to control for models' prompt sensitivity, and an empty persona setting where no persona is assigned. We find that for all models and datasets, personas show greater variability than the control setting and that some measures of persona behavior generalize across models.

==> tables/best_personas.tex <==
\begin{table}[tb]
    \setlength{\tabcolsep}{0.3em}
    \scriptsize
    \newcolumntype{P}{>{\raggedleft\arraybackslash}X}
    \begin{tabularx}{\linewidth}{lX}
        \toprule
        &Subject cat.& Best persona \\
        \midrule
        Biology & No persona \\
    Business & A person with college-level education \\
    Chemistry & A consultant \\
    Computer science & A proactive coadjutor \\
    Culture & A productive partner \\
    Economics & A financial analyst \\
    Engineering & Gustavo from brazil \\
    Geography & A social scientist \\
    Health & No persona \\
    History & An obliging supporter \\
    Law & A lawyer \\
    Math & No persona \\
    Other & A middle-class person \\
    Philosophy & A helpful assistant \\
    Physics & No persona \\
    Politics & A constructive adjunct \\
    Psychology & A psychologist \\
        \bottomrule
        \end{tabularx}
        \caption{Best persona for each MMLU subject category.}
        \label{tab:mmluSubjectBests}
\end{table}
    

\begin{table}[tb]
    \setlength{\tabcolsep}{0.3em}
    \scriptsize
    \newcolumntype{P}{>{\raggedleft\arraybackslash}X}
    \begin{tabularx}{\linewidth}{lX}
        \toprule
        &Bias cat.& Best persona \\
        Age & A nonbinary person \\
        Disability_status & A nonbinary person \\
        Gender_identity & A asexual person \\
        Nationality & A bisexual person \\
        Physical appearance & A person with neurological disorders \\
        Ethnicity & A nonbinary person \\
        Ethnicity and SES & A nonbinary person \\
        Ethnicity and gender & A nonbinary person \\
        Religion & A person with no disabilities \\
        SES & A asexual person \\
        Sexual_orientation & An uneducated person \\
        \midrule
        \bottomrule
        \end{tabularx}
        \caption{Best persona (considering accuracy) for each BBQ bias category.}
        \label{tab:BBQbiasBests}
\end{table}


==> tables/similarity_to_empty.tex <==
\begin{table*}[tb]
    \footnotesize
    \scriptsize
    \begin{tabularx}{\linewidth}{lXX}
        \toprule
         & Most similar & Least similar \\
        \midrule
        GPT-4 & an opportune helper, a resourceful associate, an effective helper, an obliging supporter, a fruitful facilitator & Francisco Franco, Adolf Hitler, Corazon Aquino, Benazir Bhutto, Jorg Haider \\
        GPT-3.5 & an efficient aid, a helpful assistant, a useful helper, an effective helper, a handy collaborator & Benito Mussolini, a comedian, a person with mental disorders, Adolf Hitler, a person with fascism ideology \\
        Mixtral & a partner, a writer, a consultant, a valuable right-hand, a model & a gay person, a person with digestive system disorders, Adolf Hitler, Benito Mussolini, Francisco Franco \\
        Zephyr & a useful helper, a helpful assistant, a reporter, an opportune helper, an efficient aid & a person with fascism ideology, a bisexual person, a homosexual person, a asexual person, a person of atheism belief \\
        Mistral-inst & a useful helper, an efficient aid, a helpful assistant, a partner, an effective helper & a homosexual person, a asexual person, a person with populism ideology, Adolf Hitler, a person with fascism ideology \\
        Gemma-7b-inst & an opportune helper, a useful helper, an efficient aid, a person with high school level education, a professor & Adolf Hitler, a person with digestive system disorders, a person with genitourinary disorders, a person with fascism ideology, a black person \\
        Gemma-2b-inst & an accommodating assistant, a helpful assistant, a social scientist, a cooperative subordinate, an obliging supporter & a person with populism ideology, Benito Mussolini, Muammar Gaddafi, Adolf Hitler, a person with fascism ideology \\
        \bottomrule
        \end{tabularx}
        \caption{The five personas most similar and least similar to the \textit{empty} persona for each model.}
        \label{tab:similarEmpty}
\end{table*}
    

==> text/discussion.tex <==
\section{Discussion}
\subsection{Takeaways}

\subsection{Further considerations}
\paragraph{Personas closest to baseline behavior}
For each model, a circle showing the spread of the persona behaviors (Cluster?). Maybe also for each dataset? 

\input{tables/similarity_to_empty.tex}


\paragraph{Performance difference between persona categories}
\begin{figure*}[tb]
  \centering
  \includegraphics[width=\linewidth]{media/performance_by_cat.pdf}
  \caption{Average persona category performance (averaged across datasets).}
  \label{fig:performanceCat}
\end{figure*}

\paragraph{Persona categories vs. control persona variability}

==> text/research_questions.tex <==
% \begin{itemize}
%   \item Previous work has shown that prompting can induce specific personalities in LLMs, influence task performance and increase biases and toxicity of generations. But some questions are still open.
%   \begin{itemize}
%       \item Task performance: it has been show that expert personas outperform non-expert personas. But how about indirect influences? Other persona types: gender, political ideology, health and socioeconomical status.  Implicit biases. I will have to distinguish this from bias runs deep paper
%       \begin{itemize}
%           \item Comparing performance of different personas on MMLU subjects and truthfulQA.
%           \item Cross-model and dataset findings
%           \item Contrary to the bias runs deep experiments, some personas can outperform empty persona basleine
%       \end{itemize}
%       \item Bias and toxicity of generations, but no impact on downstream tasks, and no measure of effect on different targets. 
%       \begin{itemize}
%           \item Comparing performance of different personas on BBQ for different bias categories and targets.
%           \item Not enough to show bias can increase.   See what kinds of bias/protected groups are most affected? generalizable across models?
%       \end{itemize}
%       \item Induce personalities, but would this affect behavior in expected way? Relate to the political compass or spinning arrow paper
%       \begin{itemize}
%           \item Compare with human annotator study. association of attitudes between humans and between personas. Association of attitudes and annotations for humans and for personas.
%       \end{itemize}
%       \item Different personas vs persona categories.
%       \begin{itemize}
%           \item Aggregate or by dataset
%           \item Which personas categories have greater variability. Does it generalize across models? Across tasks?
%       \end{itemize}
%       \item Persona vs cotrol personas. We discusses this, compare std.
%       \begin{itemize}
%           \item For each of the research questions above
%       \end{itemize}
%       \item Abstention analysis
%       \begin{itemize}
%         \item What kind of personas/datasets/models lead to abstentions. What is generalizable across those dimensions?
%       \end{itemize}
%       \item What personas are represented by the empty persona: not as reported, but based on the behavior.
%   \end{itemize}
% \end{itemize}
